RSS-based Cooperative Localization and Orientation Estimation Exploiting Directive Antenna Patterns

In this paper, we propose a factor-graph-based cooperative positioning algorithm that uses RSS radio measurements and accounts for the directivity of the antennas. This is achieved by modeling the directivity with a parametric antenna pattern and jointly estimating position and orientation of the agents. We propose two different approaches whereas the first one uses a continuous representation of the orientation state and the second one a discrete representation. We validate our proposed methods with simulations and measurements in a static sensor network with more than 900 agents in an indoor environment and show that the positioning accuracy can be improved significantly by considering the influence of orientations.

==> measModel_likelihood.tex <==
\section{Measurement Model and Likelihood}\label{sec:selection}
In this section, we describe the used RSS measurement model and the likelihood function.
%
%
%
\subsection{Measurement Model}
We model the RSS as a combination of the distance-depending path-loss and the influence of the orientation of the agents which have performed the measurements. The measurement between two nodes $i$ and $j$ is conditioned on the measurement model $M$, which is a discrete random variable, taking values of model indices $k=\{1,2,\dots,N_{\mathcal{M}}\}$. The members of the set are indicating different models and $N_{\mathcal{M}}$ being the number of models. The measurement conditioned on the model index $k$ has the form of 
\begin{align}
z_{i,j}|k &\iist = L_k(P_k,n_k,d_{i,j}) + \Psi_k(\boldsymbol{\xi}_k,\phi_{i,j},\phi_{j,i}) + n_{i,j}
\label{eq:measModelAP}
\end{align}
with the distance-depending path-loss $L_k$, the resulting change of the RSS in dependency of the orientation of the agents $\Psi_k$ and a noise term that is assumed to be Gaussian distributed as $n_{i,j}\! =\!\mathcal{N}(0,\sigma_k^2)$. In this section, we assume that the model $M\!=\!k$ as well as the model parameters are known. Different models are discussed in Section~\ref{sec:detAP}. 
The distance-depending path-loss in dB is given as
\begin{equation}
L_k(P_k,n_k,d_{i,j}) = 10\text{log} \left(10^{P_k/10} \left(\frac{d_{i,j}}{d_0}\right)^{-n_k}\right)
\label{eq:pathloss}
\end{equation}
where $n_k$ and $P_k$ are the path-loss exponent and the reference path-loss at distance $d_0$ of model $k$ respectively \cite{patwari2005locating}. The distance between the nodes is given as ${d_{i,j} = \|\mathbf{x}_j^\text{T} - \mathbf{x}_i^\text{T}\|}$ where $\|\cdot\|$ indicates the Euclidean norm. The resulting change of the measured signal strength, which depends only on the orientation of two agents, can be written as
\begin{align}
\Psi_k(\boldsymbol{\xi}_k,\phi_{i,j},\phi_{j,i}) = & \sum_{\substack{l,m \in \{i,j\} \\ l\neq m}} \bar{\Psi}_k(\boldsymbol{\xi}_k,\phi_{l,m}) 
\label{eq:2wayAP}
\end{align}
where $\phi_{i,j}$ is the angle between agent $i$ and agent $j$ with respect to the orientation $\varphi_i$ of agent $i$ and $\bar{\Psi}_k(\boldsymbol{\xi}_k,\phi)$ is a generic model of an antenna pattern.  The model parameters of the antenna pattern $\bar{\Psi}_k$ are stacked in the vector ${\boldsymbol{\xi}_k = [\xi_{k,1},\dots,\xi_{k,N_k}]^T}$ with $N_k$ being the number of parameters of the $k$th antenna pattern.
We define the angle between two nodes as ${\phi_{i,j}=\text{atan2}(y_j - y_i, x_j - x_i) - \varphi_i}$. The graphical representation of a measurement between two agents can be seen in Fig.~\ref{fig:AP}. The used antenna patterns are introduced in Section~\ref{sec:Results} and~\ref{sec:Meas_Results}.
%
%
\subsection{Likelihood} 
We define the model parameter vector for model $k$ as ${\boldsymbol{\vartheta}_k = [P_k,n_k,\boldsymbol{\xi}_k^T,\sigma_k]^T}$ that consists of the reference path-loss $P_k$ at distance $d_0$, the path-loss exponent $n_k$, the model parameters of the antenna pattern $\boldsymbol{\xi}_k$ and the shadowing standard deviation $\sigma_k$.
For a Gaussian noise model given in \eqref{eq:measModelAP}, the likelihood function can be written in the form of
\begin{equation}
f(z_{i,j}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{j},\boldsymbol{\vartheta}_k,M\!\!=\!\! k) = \frac{1}{\sqrt{2\pi \sigma_k^2}} \text{exp}\left(\frac{1}{2\sigma_k^2} (z_{i,j} - \tilde{z}_{i,j})^2  \right)
\label{eq:lhf}
\end{equation}
with
\begin{equation}
\tilde{z}_{i,j} = L_k(P_k,n_k,d) + \Psi_k(\boldsymbol{\xi}_k,{\phi}_{i,j} ,{\phi}_{j,i})
\label{eq:lhf_param}
\end{equation}
and $\boldsymbol{\theta}_i = [\mathbf{x}_i \iist\varphi_i]^\text{T} $. Note that model $k$ as well as the parameters $\boldsymbol{\vartheta}_k$ are assumed to be known which results in $f(z_{i,j}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{j})$. The different models as well as the estimation of the parameters are discussed in Section~\ref{sec:detAP}. We want to mention that in the case of discrete orientations, $\varphi_i$ is discrete and we evaluate the likelihood for every possible combination of orientations between agent $i$ and agent $j$ out of the set of discrete orientations $\mathcal{O}$.
%
\begin{figure}[t]
\centering
\input{figures/systemFigure_v2.tex}
%\input{figures/Data_cosAP_polar.tex}
\caption{This figure shows two agents and two anchors which are arbitrary orientated to one another. The centers of the nodes and the orientations are indicated by blue squares and solid blue lines, respectively. The antenna pattern $\bar{\Psi}_k(\boldsymbol{\xi}_k,\phi)$ is given in red. The dashed line indicates the measurement between two agents whereas the dotted line corresponds to measurements between anchors and agents.}
	\label{fig:AP}
\end{figure}
%
\captionsetup[subfigure]{labelformat=parens}
\begin{figure*}[t]
\centering
\subfloat[$\sigma = 1$ dB]
{\input{figures/rand2D_Result_allTypes_1dB_100agents_10anchors.tex}\label{fig:RMSE_1dB}}\hfil
\subfloat[$\sigma = 3$ dB]
{\input{figures/rand2D_Result_allTypes_3dB_100agents_10anchors.tex}\label{fig:RMSE_3dB}}\hfil
\subfloat[$\sigma = 6$ dB]
{\input{figures/rand2D_Result_allTypes_6dB_100agents_10anchors.tex}\label{fig:RMSE_6dB}}\hfil\\
\subfloat[$\sigma = 1$ dB]
{\input{figures/rand2D_angle_Result_allTypes_1dB_100agents_10anchors.tex}\label{fig:RMSE_angle_1dB}}\hfil
\subfloat[$\sigma = 3$ dB]
{\input{figures/rand2D_angle_Result_allTypes_3dB_100agents_10anchors.tex}\label{fig:RMSE_angle_3dB}}\hfil
\subfloat[$\sigma = 6$ dB]
{\input{figures/rand2D_angle_Result_allTypes_6dB_100agents_10anchors.tex}\label{fig:RMSE_angle_6dB}}\hfil\\
\pgfplotslegendfromname{legend_RMSEallRand}
\caption{Experiment 1: This figure shows the position RMSE and the RMSE of the orientation in dependency of the number of particles for 500 realizations of a scenario with 100 agents and 10 anchors for different uncertainties. %The results with known orientation are indicated in red, for continuous orientation estimation in blue, for four and eight discrete orientations in cyan and magenta respectively and no consideration of the orientation in black.}
}
\label{fig:2Drand100agents}
\end{figure*}

==> meas_likelihood_sub.tex <==
\subsection{Measurement Model}
\label{sec:measModel}
\rd{We use RSS measurements to infer position and orientation of the agents. For that case, we} model the RSS as a combination of the distance-depending path-loss and the influence of the orientation of the agents which have performed the measurements. The measurement between two nodes $i$ and $j$ is conditioned on the measurement model $M$, which is a discrete random variable, taking values of model indices $k=\{1,2,\dots,N_{\mathcal{M}}\}$. The members of the set are indicating different models and $N_{\mathcal{M}}$ being the number of models. \rd{In this section, we assume that the model $M\!=\!k$ as well as the model parameters are known. Different models are discussed in Section~\ref{sec:detAP}.} The measurement conditioned on the model index $k$ has the form of 
\begin{align}
z_{i,j}|k &\iist = L_k(P_k,n_k,d_{i,j}) + \Psi_k(\boldsymbol{\xi}_k,\phi_{i,j},\phi_{j,i}) + n_{i,j}
\label{eq:measModelAP}
\end{align}
with the distance-depending path-loss $L_k$, the resulting change of the RSS in dependency of the orientation of the agents $\Psi_k$ and a noise term that is assumed to be Gaussian distributed as $n_{i,j}\! \sim \!\mathcal{N}(0,\sigma_k^2)$. \rd{We make the common assumption that interfering multipath components, which lead to fading, as well as shadowing are only described by the noise term \cite[Section 3.9.2]{rappaport1996wireless}.} 
The distance-depending path-loss in dB is given as
\begin{equation}
L_k(P_k,n_k,d_{i,j}) = 10\text{log} \left(10^{P_k/10} \left(\frac{d_{i,j}}{d_0}\right)^{-n_k}\right)
\label{eq:pathloss}
\end{equation}
where $n_k$ and $P_k$ are the path-loss exponent and the reference path-loss at distance $d_0$ of model $k$ respectively \cite{patwari2005locating}. The distance between the nodes is given as ${d_{i,j} = \|\mathbf{x}_j^\text{T} - \mathbf{x}_i^\text{T}\|}$ where $\|\cdot\|$ indicates the Euclidean norm. The resulting change of the measured signal strength, which depends only on the orientation of two agents, can be written as \rd{the sum of the two antenna patterns evaluated at the corresponding angles $\phi_{i,j}$ and $\phi_{j,i}$ as}
%\begin{align}
%\Psi_k(\boldsymbol{\xi}_k,\phi_{i,j},\phi_{j,i}) = & \sum_{\substack{l,m \in \{i,j\} \\ l\neq m}} \bar{\Psi}_k(\boldsymbol{\xi}_k,\phi_{l,m}) 
%\label{eq:2wayAP}
%\end{align}
\rd{
\begin{align}
\Psi_k(\boldsymbol{\xi}_k,\phi_{i,j},\phi_{j,i}) = &  \bar{\Psi}_k(\boldsymbol{\xi}_k,\phi_{i,j}) + \bar{\Psi}_k(\boldsymbol{\xi}_k,\phi_{j,i}) 
\label{eq:2wayAP}
\end{align}}
where $\phi_{i,j}$ is the angle in-between agent $i$ and agent $j$ with respect to the orientation $\varphi_i$ of agent $i$ \rd{and $\phi_{j,i}$ is the angle in-between agent $j$ and agent $i$ with respect to the orientation $\varphi_j$ of agent $j$. The generic model of an antenna pattern is indicated as $\bar{\Psi}_k(\boldsymbol{\xi}_k,\phi)$.}  The model parameters of the antenna pattern $\bar{\Psi}_k$ are stacked in the vector ${\boldsymbol{\xi}_k = [\xi_{k,1},\dots,\xi_{k,N_k}]^T}$ with $N_k$ being the number of parameters of the $k$th antenna pattern.
We define the angle between two nodes as ${\phi_{i,j}=\text{atan2}(y_j - y_i, x_j - x_i) - \varphi_i}$. The graphical representation of a measurement between two agents can be seen in Fig.~\ref{fig:AP}. The used antenna patterns are introduced in Section~\ref{sec:Results} and~\ref{sec:Meas_Results}.
%
\begin{figure}[t]
\centering
\input{figures/systemFigure_v2.tex}
%\input{figures/Data_cosAP_polar.tex}
\caption{This figure shows two agents and two anchors which are arbitrary orientated to one another. The centers of the nodes and the orientations are indicated by blue squares and solid blue lines, respectively. The antenna pattern $\bar{\Psi}_k(\boldsymbol{\xi}_k,\phi)$ is given in red. The dashed line indicates the measurement between two agents whereas the dotted line corresponds to measurements between anchors and agents.}
	\label{fig:AP}
\end{figure}
%
%
\subsection{Likelihood} 
We define the model parameter vector for model $k$ as ${\boldsymbol{\vartheta}_k = [P_k,n_k,\boldsymbol{\xi}_k^T,\sigma_k]^T}$ that consists of the reference path-loss $P_k$ at distance $d_0$, the path-loss exponent $n_k$, the model parameters of the antenna pattern $\boldsymbol{\xi}_k$ and the shadowing standard deviation $\sigma_k$.
For a Gaussian noise model given in \eqref{eq:measModelAP}, the likelihood function can be written in the form of
\begin{equation}
f(z_{i,j}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{j},\boldsymbol{\vartheta}_k,M\!\!=\!\! k) = \frac{1}{\sqrt{2\pi \sigma_k^2}} \text{exp}\left(\frac{1}{2\sigma_k^2} (z_{i,j} - \tilde{z}_{i,j})^2  \right)
\label{eq:lhf}
\end{equation}
with
\begin{equation}
\tilde{z}_{i,j} = L_k(P_k,n_k,d) + \Psi_k(\boldsymbol{\xi}_k,{\phi}_{i,j} ,{\phi}_{j,i})
\label{eq:lhf_param}
\end{equation}
and $\boldsymbol{\theta}_i = [\mathbf{x}_i \iist\varphi_i]^\text{T} $. Note that model $k$ as well as the parameters $\boldsymbol{\vartheta}_k$ are assumed to be known which results in \rd{a likelihood function that depends only on the states of the nodes} $f(z_{i,j}|\boldsymbol{\theta}_{i},\boldsymbol{\theta}_{j})$. The different models as well as the estimation of the parameters are discussed in Section~\ref{sec:detAP}. 
%

